SpectralBridge: Adding High-Frequency Capability to Large Audio-Language Models

Large audio-language models (LALMs) have become highly capable on a wide range of tasks spanning speech, music, and environmental sound. However, many modern LALMs resample input audio to 16 kHz mono, making all frequencies above 8 kHz unobservable. We present SpectralBridge, a lightweight extension that gives such a model access to the 8-16 kHz band by joining low- and upper-band representations with time-aligned paired cross-frequency attention. Applied to Audio Flamingo Next, the method trains only a small adapter and rank-8 LoRA modules, while leaving the original audio encoder, audio projector, and base language model frozen. SpectralBridge improves both zero-shot transfer and downstream fine-tuning: it raises zero-shot balanced accuracy on the ESC-50 audio classification dataset from 75.5 to 90.5, and when fine-tuned on Insect-10, a 10-way insect species task we construct from InsectSet459 recordings, under the same budget as a LoRA fine-tuned baseline, it reaches 55.4 balanced accuracy against the baseline's 26.2. On a benchmark where the answer depends only on the 8-16 kHz band, it gains 30 mAP over the frozen model. Erasing the upper-band stream from the trained model removes these gains, showing that they come from the high-frequency signal itself rather than from extra tokens or the adapted prompt format.

==> nebius-palette.tex <==
\definecolor{nebiusdeepblue}{HTML}{052B42}
\definecolor{nebiuslightblue}{HTML}{F0F8FF}
\definecolor{nebiuslightblueii}{HTML}{DFEEFD}
\definecolor{nebiuslime}{HTML}{DAFF33}
\definecolor{nebiuslimeii}{HTML}{D6F34C}
\definecolor{nebiuslavender}{HTML}{C1C1FF}
\definecolor{nebiuslavenderii}{HTML}{E0E2FD}
\definecolor{nebiusviolet}{HTML}{5D52F6}

